PDDL Axioms Are Equivalent to Least Fixed Point Logic (Extended Version)

Axioms are a feature of the Planning Domain Definition Language PDDL that can be considered as a generalization of database query languages such as Datalog. The PDDL standard restricts negative occurrences of predicates in axiom bodies to predicates that are directly set by actions and not derived by axioms. In the literature, authors often deviate from this limitation and only require that the set of axioms is stratifiable. We show that both variants can express exactly the same queries as least fixed point logic. They are thus strictly more expressive than stratified Datalog, which aligns with another restriction on axioms occasionally considered in the planning literature. Complementing this theoretical analysis, we also present a compilation that eliminates negative occurrences of derived predicates from PDDL axioms.

==> mathcolor.ltx <==
%%
%% This is file `mathcolor.ltx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% mathcolor.dtx  (with options: `code')
%% 
%% The source is maintained by the LaTeX Project team and bug
%% reports for it can be opened at https://latex-project.org/bugs/
%% (but please observe conditions on bug reports sent to that address!)
%% 
%% 
%% File: mathcolor.dtx (C) Copyright 2021-2022
%%% From File: mathcolor.dtx
\def\mathcolorversion{v1.0c}
\def\mathcolordate{2022/07/25}
\ifcsname mathcolor\endcsname \endinput \fi
\ExplSyntaxOn
\seq_new:N \g__mathcolor_seq
\DeclareDocumentCommand \mathcolor { o m m }
  {
    \mode_if_math:F { \non@alpherr {\mathcolor\space} }
    \seq_gpush:No \g__mathcolor_seq \current@color
    \group_insert_after:N \use_none:n
    \IfValueTF {#1} { \color[#1]{#2} } { \color{#2} }
    #3
    \__mathcolor_scan_for_scripts:w
  }
\cs_new_protected:Npn \__mathcolor_scan_for_scripts:w
  {
    \peek_remove_filler:n
      {
        \group_align_safe_begin:
        \token_case_catcode:NnTF \l_peek_token
          {
            \c_math_subscript_token { }
            \c_math_superscript_token { }
          }
          { \__mathcolor_handle_scripts:Nw }
          {
            \token_case_meaning:NnTF \l_peek_token
              {
                \limits   { \limits }
                \nolimits { \nolimits }
                \displaylimits { \displaylimits }
              }
              {
                \group_align_safe_end:                          % case 4
                \__mathcolor_scan_for_scripts:w \use_none:n
              }
              {
                \token_if_eq_meaning:NNTF \l_peek_token '
                  {
                    \__mathcolor_handle_scripts:Nw ^
                    \c_group_begin_token
                      \exp_after:wN \prim@s \use_none:n
                  }
                  {
                    \group_align_safe_end:                      % case 1
                    \reset@color
                    \seq_gpop:NN \g__mathcolor_seq \current@color
                  }
              }
          }
      }
  }
\cs_new_protected:Npn \__mathcolor_handle_scripts:Nw #1
  {
    #1 \c_group_begin_token \c_group_begin_token
    \seq_get:NN \g__mathcolor_seq \current@color
    \set@color
    \group_insert_after:N \c_group_end_token
    \group_insert_after:N \__mathcolor_scan_for_scripts:w
    \peek_remove_filler:n
      {
        \token_if_eq_meaning:NNTF \l_peek_token \c_group_begin_token
          {
            \group_align_safe_end:                              % case 2
            \peek_catcode_remove:NT \c_group_begin_token { }
          }
          {
            \exp_after:wN \group_align_safe_end:                % case 3
              \use_ii_i:nn \c_group_end_token
          }
      }
  }
\ExplSyntaxOff
%%%%%%%%%%%%%%%%
\endinput
%%
%% End of file `mathcolor.ltx'.

